Characterizing Off-path SmartNIC for Accelerating Distributed Systems

SmartNICs have recently emerged as an appealing device for accelerating distributed systems. However, there has not been a comprehensive characterization of SmartNICs, and existing designs typically only leverage a single communication path for workload offloading. This paper presents the first holistic study of a representative off-path SmartNIC, specifically the Bluefield-2, from a communication-path perspective. Our experimental study systematically explores the key performance characteristics of communication among the client, on-board SoC, and host, and offers insightful findings and advice for designers. Moreover, we propose the concurrent use of multiple communication paths of a SmartNIC and present a pioneering guideline to expose new optimization opportunities for various distributed systems. To demonstrate the effectiveness of our approach, we conducted case studies on a SmartNIC-based distributed file system (LineFS) and an RDMA-based disaggregated key-value store (DrTM-KV). Our experimental results show improvements of up to 30% and 25% for LineFS and DrTM-KV, respectively.

==> dpu-v1.tex <==
\section{Off-path SmartNIC Performance Analysis}
\label{sec:dpu}

This section presents our insights in best-utilizing off-path {\snic}. 
We first briefly summarize known insights from existing {\snic} studies~\cite{DBLP:journals/corr/abs-2105-06619, thostrupdbms, ipipe, linefs}, 
which turn valuable but insufficient in guiding applications to understand the architecture implications 
of off-path NICs and their offloading bottlenecks. 

\subsection{Current findings of off-path SmartNIC}
\label{sec:dpu-related}

%Known performance characteristics of {\dpu} are:  

\begin{itemize}[wide, labelindent = 0pt, topsep = 1ex]
  \item \textbf{Wimpy computing power}. Due to power constraints, 
  it is well known that 
  the offloading computing power on {\snic}, 
  i.e., CPU speed (2.75GHz vs. 3.6GHz), 
  number of cores (8 vs. 12) and memory access latencies, 
  are slower/smaller than the host~\cite{ipipe, DBLP:journals/corr/abs-2105-06619, linefs, thostrupdbms}. 
  % This challenges developers to choose what to offload on {\snic}s. 
  As a result, 
  SoC cores cannot fully utilize the NIC cores to send packets to the others~\cite{ipipe, DBLP:journals/corr/abs-2105-06619}

  \item \textbf{NIC is faster in reading the onboard DRAM. }
  Thostrup~{\etal}~\cite{thostrupdbms} found that 
  the READ are faster when accessing the SoC memory than accessing the host. 
  Table~\ref{tab:lat-data} shows the latency results on different networking primitives
  and confirms their results (SNIC-H vs. SNIC-S: 2.3 vs. 2 $\mu$s).
  They attribute the performance improvements to the ``closer'' placement of NIC cores to the onboard DRAM.
  Our investigation reveals what ``closer'' means:
  the NIC cores can save one PCIe data path for accessing its onboard DRAM (\textsection{\ref{sec:dpu-perf-wo-offloading}}). 

  \item \textbf{Slow communication between SoC and host.}
  It is well known that accessing the host memory at the NIC-side via PCIe is slow,  
  but the accesses from the off-path SoC are even slower than RNICs or on-path NICs (in terms of latency) 
  because they wrap the PCIe traffic with RDMA to simplify programming~\cite{ipipe}. 
  We further discover that leveraging RDMA incurs unexpected performance bottleneck (\textsection{\ref{sec:dpu-perf-w-offloading}}).
\end{itemize}

\input{latency-tab.tex}

\subsection{Architecture implications of host networking}
\label{sec:dpu-perf-wo-offloading}

We now present our findings of the performance implications of off-path SmartNIC, 
focusing on its networking performance as its computation capability has been extensively studied in the literature. 
\iffalse
In particular, 
this section first aims to answer the following two questions: 

\begin{enumerate}[leftmargin=*,leftmargin=5pt,itemindent=7pt]
  \item What is the impact to the host networking compared to a NIC without offloading support?
  \item What are the performance benefits {\snic} can bring? 
\end{enumerate}

\noindent
We leave the investigation of the communication performance between SoC and host into the next section. 
\fi

For the first question, 
our main finding is that systems using the {\snic}s suffer 
a phenomenon we called \emph{heterogeneous performance degradations}. 
Specifically, 
compared to the NIC with the same specification of the NIC core,
the off-path architecture would cause performance degradations when communicating with the host,
but degradations are heterogeneous: 
some workloads suffer more overhead but some are unaffected. 

\vspace{5pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {1. {\snic} has a higher latency when communicating with the host}.}
}
\vspace{2pt}

Table~\ref{tab:lat-data} presents the latencies of a single client issuing 
different RDMA requests to different NICs. 
We particularly focus on comparing {\snic} (SNIC-H) and CX6 
because their internal NIC cores are the same~\cite{bluefield-2}. 
The results show that the latencies of READ, WRITE and SEND/RECV increase 22\%, 25\% and 26\% 
when extending the RNIC to {\snic}. 
These numbers are even high than an old generation of RNIC (CX4). 
We suspect the inflated latency of {\snic} is due to the extra PCIe switch that resides between the NIC and the host, 
plus the additional hardware circuits to support offloading. 

\vspace{5pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {2. Outbound requests from {\snic} is \TODO{xx}.}
}}
\vspace{2pt}

\begin{figure}[!t]
    \hspace{-3mm}
%    \centering
    \includegraphics[left, scale=1.18]{data/micro/inbound.pdf}  \\[3pt]
        \begin{minipage}{1\linewidth}
          \caption{\small{%
            Inbound RDMA throughput and bandwidth of different NICs. 
            The InfiniBand limit of {\snic} and RDMA is 200Gbps.
            }}
        \label{fig:motiv-dpu-perf}
        \end{minipage} \\[-10pt]
    \end{figure} 

\vspace{5pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {3. Inbound READ from {\snic} suffers degraded throughput for small payloads. }
}
}
\vspace{2pt}

\fig{fig:motiv-dpu-read-perf} shows the inbound READ throughput 
with different RDMA request payloads. 
We report the peak throughput/bandwidth of a single NIC 
by increasing the number of clients communicating with the NIC until it is saturated. 
Due to the lack of machines in PCIe4 cluster, 
we also deploy clients at the PCIe3 cluster by sending requests to the {\snic} hosted on PCIe4. 

\begin{figure}[!t]
  \centering    
  \includegraphics[scale=1.05]{figs/network-slowdown.pdf}  \\[5pt]
  \begin{minipage}{1\linewidth}
  \caption{\small{%
    The execution flows of READ and WRITE on (a) {\snic} and (b) RNIC.
  }}
  \label{fig:dpu-slowdown}
  \end{minipage} %\\[-10pt]
\end{figure}

On PCIe4, RDMA is 13--21\% faster than {\snic} (SNIC) 
for READ smaller than 256B with the same NIC cores (ConnectX-6). 
This gap is due to the fact that READ must additionally pass the switch twice in {\snic}. 
As shown in \fig{fig:dpu-slowdown}, 
the NIC processing unit first issues a PCIe request to the switch to read the memory, 
whose payload is transferred back to the switch.
This could significantly inflate the processing pipeline of sending and receiving DMA requests 
in the NIC cores\footnote{\footnotesize{Though 
detailed analysis requires proprietary/confidential NIC manuals unavailable to us.}}.
On large payloads ($\geq$ 256B), 
{\snic} is similar to RDMA because the overhead of transferring the data will dominate 
the performance. 

On PCIe3, we observe a similar phenomenon: 
for smaller payloads ($\leq$64B), RDMA is 9--28\% faster, 
even RDMA on PCIe3 uses an old RNIC (ConnectX-4 vs. ConnectX-6).
Thanks to the more powerful RNIC, 
{\snic} is 17--56\% faster for payloads larger than or equal to 64B,
as large payloads are less affected by the extra latency introduced by {\snic} hardware.
A final takeaway from PCIe3 is that the old generation of PCIe fails to saturate the new {\snic}s. 
PCIe3.0 x16 only provide 128Gbps peak inbound bandwidth. 
Therefore, {\snic} can only achieve 103Gbps for 1024B payload. 

\subsection{Architecture implications of SoC networking}
\label{sec:dpu-perf-soc}

We refer to SoC networking as its capability to communicating with the others. 
\TODO{xx}

\subsection{Communications between SoC and host}
\label{sec:dpu-perf-w-offloading}

\[ Peak(O_{s}) = Peak(R) = max(2 * N_{bd}, 2 * P_{bd}) \]

\[ Peak(O_{c}) = P_{bd} \]

\paragraph{Impliciations.}
\TODO{xx}

==> dpu-v2.tex <==
\section{Off-path SmartNIC Performance Analysis}
\label{sec:dpu}

This section presents our insights in best-utilizing off-path {\snic}, 
focusing on its networking performance as its computation capability has been extensively studied 
in the literature summarized in the previous section. 
We discuss three aspects of {\snic} networking performance in this section:
the efficiency of host interacting with the others via {\snic}, 
the efficiency of SoC on the {\snic} interacting with others except for the host 
and the performance bottleneck of SoC communicating with the host (and vice versa). 

\subsection{Performance implications for host networking}
\label{sec:dpu-host-networking}

Treating {\snic} as a vanilla RNIC suffers a foundational \emph{performance degradation}: 
its performance (in terms of access latencies and request throughput) 
is weaker than the same standard of RNIC. 
To show this, we conducted a series of microbenchmarks comparing {\dpu} with ConnectX-6.
These comparisons best illustrate the performance tax paid by extending an RNIC to {\snic},
because {\dpu} uses the same NIC cores as ConnectX-6~\cite{bluefield-2}. 

\begin{figure}[!t]
    \centering    
    \includegraphics[scale=1.0]{figs/network-slowdown.pdf}  \\[5pt]
    \begin{minipage}{1\linewidth}
    \caption{\small{%
      The execution flows of READ and WRITE on (a) {\snic} and (b) RNIC.
    }}
    \label{fig:dpu-slowdown}
    \end{minipage} %\\[-10pt]
  \end{figure}

\paragraph{Access latency. }
We first measure the latencies of CLI communicates with SRV via different NICs. 
Table~\ref{tab:lat-data} shows that 
CLI suffers a \TODO{xx, xx and xx} latency increases for 
READ, WRITE and SEND+RECV
when attaches {\dpu} to SRV compared to ConnectX-6, respectively. 
The increased latency is mainly due to the extra PCIe switch
added between the NIC cores and host, as illustrated in {\fig{fig:dpu-slowdown}}. 
READ suffers a larger (\textasciitilde2X) latency increases than WRITE (\TODO{xx}X). 
This is because the data path of READ must pass the PCIe switch twice: 
READ internally issues a PCIe READ to the host, which contains a request packet and completion packet. 
On the other hand, 
the WRITE can skip the completion of the PCIe write~\cite{pcie-talk, adr}. 


\begin{figure}[!t]
  \hspace{-3mm}
%    \centering
  \includegraphics[left, scale=1.00]{data/micro/inbound.pdf}  \\[3pt]
      \begin{minipage}{1\linewidth}
        \caption{\small{%
          Inbound RDMA throughput and bandwidth of different NICs. 
          The InfiniBand limit of {\snic} and RDMA is 200Gbps.
          }}
      \label{fig:motiv-dpu-perf}
      \end{minipage} \\[-10pt]
  \end{figure} 

\paragraph{Inbound requests throughput. }
A direct impact of the increased access latency is the degraded throughput for inbound requests, 
\ie{the throughput of different clients sending RDMA requests to the host}. 
{\fig{fig:motiv-dpu-perf}} shows \TODO{xx}. 

\begin{figure}[!t]
  \hspace{-3mm}
%    \centering
  \includegraphics[left, scale=1.00]{data/micro/outbound.pdf}  \\[3pt]
      \begin{minipage}{1\linewidth}
        \caption{\small{%
          Outbound RDMA performance of different NICs. \TODO{This figure is just a placeholder.}
          }}
      \label{fig:motiv-dpu-perf-out}
      \end{minipage} \\[-10pt]
  \end{figure} 

\paragraph{Outbound requests throughput. }

%% TBD: currently not focus on this
% \paragraph{Cache-miss penalties. }

\paragraph{Implications.}

\iffalse
\begin{figure*}[!t]
\centering
\begin{minipage}{.3\textwidth}  
  \vspace{-5pt}
  \hspace{-15pt}
  \includegraphics[left, scale=1]{figs/bottleneck.pdf}
\end{minipage}%
\begin{minipage}{.33\textwidth}
  \hspace{-10pt}
  \includegraphics[left, scale=1]{data/micro/bottleneck-separate.pdf}
\end{minipage}
\begin{minipage}{.33\textwidth}
  \hspace{5pt}
  \includegraphics[scale=1,right]{data/micro/bottleneck-separate.pdf}
\end{minipage}    \\[5pt]
\begin{minipage}{1\textwidth}
    \caption{\small{%
          \TODO{The data here is a placeholder. }
          }}
      \label{fig:offloading-bottlenecks}
      \end{minipage} \\[-10pt]
\end{figure*} 
\fi

\subsection{Performance implications of separate offloading}
\label{sec:dpu-soc-networking} 

Separate offloading provides the following benefits for distributed applications.
First, inbound requests to the SoC is typically faster than the host or even faster than RDMA. 
Second, issuing requests to the SoC and host simultaneously can mitigate the host network degradation. 
Finally, it can best utilize the PCIe and network bandwidth for offloading. 

\paragraph{Inbound requests throughput.} 


\paragraph{Outbound requests throughput.}


\paragraph{Offloading bottlenecks.}
As shown in {\fig{fig:offloading-bottlenecks}} (a), 
the bottleneck of communicating with SoC is determined by the 
limit of the network and PCIe (PCIe1), 
because the traffic only flows between these two components. 
On typical NICs, the internal PCIe limit is larger than the network
(e.g., the unidirectional bandwidth of {\dpu} is 200Gbps and 256Gbps for network and PCIe, respectively). 
Therefore, the bottleneck of a single request communicating with the SoC is bottlenecked by the network.  
{\fig{fig:offloading-bottlenecks}} (b) shows the result of Inbound SNIC-S READ. 
With \TODO{xx} CLIs, we can saturate the network limit for large payload (4096B), 
achieving 200Gbps. 
Note that we skip other requests type since they have the same bottleneck.

A more interesting bottleneck to explore is the maximum bandwidth 
of the system of separate offloading, 
i.e., the CLIs communicate with the host and the SoC simultaneously. 
Our finding is that the data flow direction of different requests matters. 
The direction means how data flows over the PCIe or the network. 
As shown in {\fig{fig:offloading-bottlenecks}} (a), 
the data of Inbound SNIC-S READ (\ding{192}) flows \emph{out} of the PCIe and network, 
while the data of Inbound SNIC-H WRITE (\ding{193}) flows \emph{in} to the NIC. 
Therefore, the above two requests are in a different direction. 
On the other hand, Inbound SNIC-H READ (\ding{194}) has the same direction with \ding{192}. 

Denote the bandwidths of network and PCIe are $N_{bd}$ and $P_{bd}$, respectively. 
The maximum bandwidth of separate offloading $Peak(O_{s}) = max(2 * N_{bd}, 2 * P_{bd})$, 
which can be achieved only when the requests to the SoC and the host are at different directions. 
When requests are in different direction, they can enjoy the full bidirectional bandwidth of PCIe and network~\cite{rdma-bidirectional}, 
doubling the achievable bandwidth limit.  
As shown in {\fig{fig:offloading-bottlenecks}} (b), 
Inbound SNIC-S READ + Inbound SNIC-H WRITE can reach 400Gbps,
while Inbound SNIC-S READ + Inbound SNIC-H READ can only achieve 200Gbps.
We omit the results of other request patterns since they are similar. 


\paragraph{Implications.}
1. Networking to SoC is fast. 
2. Hybrid is better.

\subsection{Communications between SoC and host}
\label{sec:dpu-soc-host-networking}

\[ Peak(O_{c}) = P_{bd} \]

\paragraph{Implications.}

==> dpu.tex <==
\section{Analysis of Off-path SmartNIC}
\label{sec:dpu}

%\vspace{5pt}
With the help of on-board computing power (ARM) and DRAM, 
{\snic} opens opportunities to offload transaction processing 
to mitigate drawbacks of RDMA for transactions. 
Nevertheless, as we have mentioned in the introduction, 
there lacks a deep understanding of the \emph{inbound} networking performance of {\snic} 
and how the offloading traffic interacts with the normal traffic. 
Our analyses reveal the following new observations for {\snic}: 

\begin{itemize}[leftmargin=*,leftmargin=5pt,itemindent=7pt]
  \item {\snic} exhibits \emph{heterogeneous performance degradation} 
  to the in-bound network performance compared with RNIC, 
  even without considering the offloading traffic. 
  \item The impact of offloading traffic on the host is also heterogeneous: 
  some may huge, others maybe negligible. 
\end{itemize}

\noindent
As a result, naively offloading transactions to {\snic} may yield 
even poorer performance than RDMA (see \textsection{\ref{sec:design}}). 
We first explore the details of our findings in this section.

\input{hardware-tab.tex} 

\paragraph{Testbed.}  
We use two local rack-scale clusters for all the experiments, 
representing old configurations of RDMA-capable clusters (PCIe3) and recent configurations (PCIe4). 
Table~\ref{tab:hardware-info} presents the detailed setups of the two clusters and the in-measured {\snic}s. 
For {SNIC}-related evaluation, 
we will replace the RNICs to the {\snic}s for each cluster.
Machines in each cluster are connected via one Mellanox SB7890 100Gbps InfiniBand Switch. 
Note that this won't degrade the network performance for 200Gbps RNIC or {\snic}:
 both NICs have two 100Gbps ports. 

% \paragraph{Terminology}.
% Like existing works on analysing the performance of RDMA, 
% \TODO{Xx}

\subsection{Heterogeneous downgrades to host}
\label{sec:dpu-downgrade}

\input{latency-tab.tex}

This section analyzes the impact of off-path {\snic} architecture on hosting networking 
without offloading,
which we show is non-negligible. 
Specifically, 
the internal hardware circuits to support computing units and PCIe switch 
causes extra hops in the {\snic}'s networking processing pipeline.
%\fig{fig:dpu-slowdown} summarizes the impact to RDMA READ/WRITE. 
%We omit two-sided RDMA because the execution flow of sending a packet 
%is similar to WRITE~\cite{DBLP:conf/usenix/KaliaKA16}.
A direct impact is the added latencies to each RDMA request (see Table~\ref{tab:lat-data}).  
On PCIe4 cluster, 
the latencies of 8B {\snic} READ is 21\% higher than RDMA using the same RNIC. 
The added latencies will further bring significant performance downgrades to the peak throughput
especially for small payloads (large payloads are less affected due to their longer processing time), 
but we found that the impact is \emph{heterogeneous}:
READ suffers a significant performance downgrade but WRITE is unaffected. 
More specifically: 
\vspace{5pt}

\begin{figure}[!t]
  \centering    
  \includegraphics[scale=1.05]{figs/network-slowdown.pdf}  \\[5pt]
  \begin{minipage}{1\linewidth}
  \caption{\small{%
    The execution flows of READ and WRITE on (a) {\snic} and (b) RNIC.
  }}
  \label{fig:dpu-slowdown}
  \end{minipage} %\\[-10pt]
\end{figure}

\begin{figure}[!t]
    \hspace{-3mm}
%    \centering
    \includegraphics[left, scale=1.18]{data/micro/basic-read.pdf}  \\[3pt]
        \begin{minipage}{1\linewidth}
          \caption{\small{%
            Inbound READ throughput and bandwidth of different NICs, 
            and the InfiniBand limit of {\snic} (200Gbps).
            }}
        \label{fig:motiv-dpu-read-perf}
        \end{minipage} \\[-10pt]
    \end{figure} 

%\vspace{1.mm}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {1. {\snic} READ to host is slower than RDMA}.}
}

\vspace{5pt}
\fig{fig:motiv-dpu-read-perf} shows the inbound READ performance 
with different RDMA request payloads. 
We report the peak throughput/bandwidth of a single NIC 
by increasing the number of clients communicating with the NIC until it is saturated. 
Due to the lack of machines in PCIe4 cluster, 
we also deploy clients at the PCIe3 cluster by sending requests to the {\snic} hosted on PCIe4. 

On PCIe4, RDMA is 13--21\% faster than {\snic} (SNIC) 
for READ smaller than 256B.
Note that the internal NIC used by {\snic} is the same as RDMA (ConnectX-6), 
showing that {\snic} has a performance gap with RDMA. 
We attribute this gap to the fact that READ must additionally pass the switch twice:
as shown in \fig{fig:dpu-slowdown}, 
the NIC processing unit first issues a PCIe request to the switch to read the memory, 
whose payload is transferred back to the switch. 
Passing the switch extends the NIC's processing time for the READ request, 
causing throughput degradation.\footnote{\footnotesize{A 
detailed analysis requires proprietary/confidential NIC manuals, which are unavailable to us.}}
On large payloads ($\geq$ 256B), 
{\snic} is similar to RDMA because the overhead of reading the data will dominate the transfer time. 

On PCIe3, we observe a similar phenomenon: 
for smaller payloads ($\leq$64B), RDMA is 9--28\% faster, 
even RDMA on PCIe3 uses an old RNIC (ConnectX-4 vs. ConnectX-6).
Thanks to the more powerful RNIC, 
{\snic} is 17--56\% faster for payloads larger than or equal to 64B,
as large payloads are less affected by the extra latency introduced by {\snic} hardware.
A final takeaway from PCIe3 is that the old generation of PCIe fails to saturate the new {\snic}s. 
PCIe3.0 x16 only provide 128Gbps peak inbound bandwidth. 
Therefore, {\snic} can only achieve 103Gbps for 1024B payload. 
\vspace{5pt}

\begin{figure}[!t]
  \hspace{-3mm}
%  \centering
  \includegraphics[left, scale=1.18]{data/micro/basic-write.pdf}  \\[3pt]
      \begin{minipage}{1\linewidth}
        \caption{\small{%
          Inbound WRITE throughput and bandwidth of different NICs, 
          and the InfiniBand limit of {\snic} (200Gbps).
        }}
      \label{fig:motiv-dpu-write-perf}
      \end{minipage} \\[0pt]
  \end{figure}   

%\vspace{1.mm}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {2. {\snic} WRITE to host is as fast as RDMA}.}
}  

\vspace{5pt}
\fig{fig:motiv-dpu-read-perf} shows the inbound WRITE performance using the same setup as READ. 
Unlike READ, SNIC has similar performance as RDMA (except for payloads smaller than 64B) on PCIe4 
and is 26--70\% faster on PCIe3. 
Under the same NIC (PCIe4), WRITE is less affected by the increased PCIe latency 
due to its different processing pattern shown in \fig{fig:dpu-slowdown}. 
WRITE internally issues a PCIe WRITE to the host, which will not generate an acknowledgment packet~\cite{pcie-talk}. 
Hence, NIC may finish the processing without waiting for the WRITE to complete~\cite{adr}. 
Therefore, the extra latencies added by the PCIe switch are not on the critical path of WRITEs. 
The latency results in Table~\ref{tab:lat-data} confirms this: 
WRITE to {\snic} is 1.8$\times$ faster than READ 
while for RDMA the difference is negligible. 
For PCIe3, {\snic} is faster due to adopting a newer generation of NIC inside.
\vspace{5pt}
  
\begin{figure}[!t]
  \hspace{-3mm}
%      \centering
      \includegraphics[left, scale=1.18]{data/micro/basic-rpc.pdf}  \\[3pt]
          \begin{minipage}{1\linewidth}
            \caption{\small{%
              Inbound two-sided throughput and bandwidth of different NICs, 
              and the InfiniBand limit of {\snic} (200Gbps).   
              }}
          \label{fig:motiv-dpu-rpc-perf}
          \end{minipage} \\[0pt]
      \end{figure} 
  

%\vspace{1.mm}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {3. {\snic} Two-sided to host is also slower than RDMA}.}
}  

\vspace{5pt}
Two-sided RDMA also suffers a downgrade performance (for the same NIC) 
due to the increased latency caused by {\snic} (see Table~\ref{tab:lat-data}). 
\fig{fig:motiv-dpu-rpc-perf} presents the in-bound two-sided performance on PCIe4 and PCIe3, respectively.
Each client sends ping-pong requests with various payloads to the server. 
The server utilizes all the CPUs on the NIC's attached sockets to handle requests. 
On PCIe4, SNIC can only achieve 70--93\% of the peak throughput of RDMA. 
On PCIe3, SNIC is 9--37\% faster thanks to the new generation of RNIC. 

%Unlike one-sided RDMA whose performance solely depends on the NIC, 
%the server's CPU available for processing the messages is also worth noting. 
%In the case of the distributed transaction, xxx. 


\vspace{5pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {4. One-sided RDMA to the {\snic} is fast except for two-sided RDMA}.}
}  

\vspace{5pt}
The efficiency of communicating with {\snic}'s onboard computing resources 
(we term \emph{ARM} in this paper) 
is also critical to the applications trying to utilize {\snic}. 
We also measured its performance (SNIC-A) in \fig{fig:motiv-dpu-read-perf}--\ref{fig:motiv-dpu-rpc-perf}. 
Our analyses reveal the following new observations for {\snic}: 

\begin{figure*}[!t]
  \hspace{2mm}
%      \centering
      \includegraphics[left, scale=1.18]{figs/network-conflict.pdf}  \\[10pt]
          \begin{minipage}{1\linewidth}
            \caption{\small{%
              An illustration of how networking requests to (inbound) and from (outbound) {\snic} 
              can interfere with the host networking.               }}
          \label{fig:network-conflict}
          \end{minipage} \\[-10pt]
      \end{figure*} 

First, READ to ARM is not affected by the performance downgrade introduced by {\snic}
and is even faster than RDMA. 
As shown in \fig{fig:motiv-dpu-read-perf}, 
SNIC-A is 5--51\% and 18--60\% faster than SNIC and 
11--24\% and 16--95\% faster than RDMA on PCIe4 and PCIe3, respectively.
Our suspicion is that the onboard PCIe switch can access the onboard DRAM 
with a faster internal protocol other than PCIe.  
For example, the bluefield SmartNIC only provides two counters
for PCIe0 ({\snic}->Host) and PCIe1 (RNIC -> PCIe switch) shown in \fig{fig:smartnic},
not PCIe switch -> ARM's DRAM~\cite{bluefield-counter}. 
The empirical latency results in Table~\ref{tab:lat-data} match our suspicion: 
READ to ARM has a lower latency than WRITE.
Note that reading {\snic}'s on-board DRAM still has a higher latency 
than reading host with RDMA (1.99$\mu$s vs. 1.89$\mu$s).
We attribute it to the added circuit complexity of SmartNIC.

Second, WRITE to ARM has nearly the same performance as RDMA and SNIC (see \fig{fig:motiv-dpu-write-perf}),
demonstrating that the bottleneck of the WRITE is the NIC's processing power.

Finally, two-sided RDMA to ARM suffers a significant performance downgrade compared 
with SNIC and RDMA (see \fig{fig:motiv-dpu-rpc-perf}). 
This is because power and hardware restrictions typically 
weaken the onboard computing resources of {\snic}. 
%Specifically, our evaluating {\snic} has eight ARM Cortex-A72 2.75GHz cores, 
%while the host is equipped with twelve 3.6GHz cores (PCIe4). 
As a result, posting a two-sided request is \TODO{xx} slower than the host.
Therefore, the on-board CPU (ARM) is the bottleneck (not the network). 
%Though batching can mitigate the posting overhead~\cite{DBLP:conf/usenix/KaliaKA16}, 
%we disable batching in this experiment 
%because it is not suitable for online transaction processing. 

\subsection{Heterogeneous interferences of {\snic}}
\label{sec:dpu-interference}

Traffic from/to {\snic}'s on-board DRAM/CPU competes with 
NIC's processing power, NIC bandwidth and host's PCIe bandwidth from/to host, 
causing performance interferences. 
We found the degree of interferences is different considering the request patterns.
Therefore, we should carefully avoid them in utilizing {\snic}. 

To better understand behaviors of requests from/to {\snic}, 
we categorize them as follows (see \fig{fig:network-conflict}--\ref{fig:network-directions}):  \\[-20pt]

\vspace{5pt}
\begin{itemize}[wide, labelindent = 0pt, topsep = 1ex]
  \setlength\itemsep{0em}
  \item[\texttt{Inbound.}] Requests that are sent to the ARM. 
  Examples include a client sending a READ request to read the ARM's memory.   
  \item[\texttt{Outbound.}]  Requests initiated by the ARM, 
  e.g., send a WRITE to write the memory of a remote server. 
  \item[\texttt{Host conflict.}] An inbound/outbound request to/from ARM communicates with the host. 
  For example, the ARM can issue an outbound READ to read the host memory.  
\end{itemize}

\iffalse
\begin{figure}[!t]
  \hspace{-3mm}
%      \centering
      \includegraphics[left, scale=1.0]{figs/network-directions.pdf}  \\[15pt]
          \begin{minipage}{1\linewidth}
            \caption{\small{%
              An illustration of the offloading network packet directions to and from {\snic}.             }}
          \label{fig:network-directions}
          \end{minipage} \\[-20pt]
      \end{figure}
\fi       

Besides the request types described above, 
we found the \emph{traffic direction}---how packet flows into the NIC 
is also an important factor, as shown in \fig{fig:network-directions}:    

\vspace{3pt}
\begin{itemize}[wide, labelindent = 0pt, topsep = 1ex]
  \setlength\itemsep{0em}
  \item[\texttt{Same.}] The packets to/from ARM are aligned with
  the packets to/from the host. 
  Note that the packet direction depends on the request type (READ or WRITE), 
  not inbound or outbound. 
  For example, an outbound READ from ARM can have the same direction as an inbound WRITE to host. 
  \item[\texttt{Different.}]  The packets to/from ARM are in a different direction as host, 
  e.g., an inbound ARM READ vs. an inbound host WRITE.
\end{itemize}

\vspace{5pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {5. For small offloading requests, the host networking favors inbound request over 
  outbound over host conflict, and WRITEs are preferred over READs.
}}}
\vspace{5pt}

For small RDMA requests(e.g., < 512B) to/from ARM, 
the degree of inferences is determined by how they compete for the NIC's processing power with the host. 
It is well known that different types of requests consume different RNIC processing capabilities~\cite{herd}. 
Specifically, inbound requests are faster than outbound ones,
and WRITE is faster than READ. 
For example, inbound READ only requires a DMA read plus a packet transmission, 
while outbound READ needs an MMIO, send a packet, receive a packet and a DMA WRITE. 
We found these findings still hold for {\snic} when considering offloading interferences:
the interferences from inbound request is typically smaller than outbound ones. 
Meanwhile, the interferences are small when considering WRITEs. 

\iffalse
\begin{figure}[!t]
  \hspace{-3mm}
%      \centering
      \includegraphics[left, scale=1.18]{data/micro/network-conflict.pdf}  \\[3pt]
          \begin{minipage}{1\linewidth}
            \caption{\small{
            Impact of a constant 8M reqs/sec offloading traffic from/to ARM 
            on host networking. 
              }}
          \label{fig:network-conflict-data}
          \end{minipage} \\[-10pt]
      \end{figure}  
\fi       

We measured the impact of different requests in \fig{fig:network-conflict-data} 
conducted on the PCIe4. 
We omit the results on PCIe3 because they are the same. 
To make a fair comparison, 
we use an open-loop harness to control a fixed 8M requests/sec traffic from/to ARM. 
Before adding the interferences, we use 2 clients to saturate the host's performance (Host). 
First, we observe that inbound requests bring slightly larger overhead than outbound ones. 
In the top-left figure where the host requests are READ while ARM also uses READ, 
+ARM(Inbound) incurs 8--10\% slowdown to host for payloads within 10--128 
while +ARM(Outbound) incurs 15--20\% slowdown. 
Nevertheless, the differences become smaller when considering WRITEs. 
For example, 
in the right bottom plot we can see both +ARM(Inbound) and Outbound would incur 
a similar 1--9\% slowdown.

Another important observation is that the host conflict mode is always slower than the others. 
In the top left plot of \fig{fig:network-conflict-data}, 
+ARM(Host conflict) incurs a 50--60\% slowdown to host READ for payloads 16--128B.
This is because it not only competes for network processing power with the host 
but also competes PCIe bandwidth, as shown in \fig{fig:network-conflict} (c).

\iffalse
\begin{figure}[!t]
  \hspace{-3mm}
%      \centering
      \includegraphics[left, scale=1.18]{data/micro/traffic-direction.pdf}  \\[5pt]
          \begin{minipage}{1\linewidth}
            \caption{\small{
              Impact of the offloading traffic on host considering 
              the conflicting traffic directions:
              \textbf{Same}: the packet directions are the same for host and ARM.
              \textbf{Different}: the packet directions are different. 
            }}
          \label{fig:network-direction-same}
          \end{minipage} \\[-5pt]
      \end{figure}   
\fi


\vspace{8pt}
\noindent \fbox{
\parbox{0.96\linewidth}{
\noindent {6. For large offloading requests, 
the host networking favors a different direction of ARM.
}}}
\vspace{3pt}      

For larger payloads (e.g., 1024B), 
the network and PCIe bandwidth will be the performance bottleneck. 
We observe an interesting phenomenon: 
If the direction of the packet from/to ARM is different from host,
the host bandwidth will not be affected by ARM. 
\fig{fig:network-direction-same} plots the impact of added ARM traffic 
on the host networking performance. 
We use the same setup as the previous experiment and the inbound load for ARM
 (the differences in requests are negligible on large payloads). 
We only describe the results when the networking is READ to host (a), 
i.e., other clients reading from the host,
the WRITE results are the same. 
When adding READ to ARM (+ARM(Same)), 
the host bandwidth will decrease to 100Gbps for larger than 512B payloads 
as the ARM share half of the overall bandwidth (200Gbps). 
In comparison, adding WRITE to ARM  (+ARM(Same)) does not affect the host, 
and the {\snic} can achieve nearly 400Gbps bandwidth in total. 
The reason behind this finding is that the InfiniBand and PCIe bandwidth is 
bidirectional~\cite{rdma-bidirectional}. 
Therefore, packets from different directions can share the same link simultaneously 
without losing performance. 

==> hardware-tab.tex <==
\begin{table}[!t]  
    \vspace{2.2mm}
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
        Measurement clusters.  
        }}}        
        \label{tab:hardware-info}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
        \small{            
          \resizebox{.48\textwidth}{!}{%
          \begin{tabular}{p{0.3\linewidth}p{0.65\linewidth}}
            \toprule
            \textbf{Cluster Name}       & \textbf{Hardware configurations}                                                                                             \\ \hline
            PCIe3      & \TODO{num} machines, each with ConnectX-4 (CX4, 1$\times$ 100Gbps InfiniBand port), PCIe 3.0 $\times$16 (\red{128Gbps}), Intel Xeon E5-2650 v4 (12 cores, 2.2GHz)    \\
            PCIe4      & \TODO{num} machines, each with ConnectX-6 (CX6, 2$\times$ 100Gbps InfiniBand ports), PCIe 4.0 $\times$16 (\red{256Gbps}), Intel Xeon Gold 5317 v4 (12 cores, 3.6GHz) \\
            \bottomrule            
            \end{tabular}              
        }
        } % end small
\end{table}   

==> latency-tab.tex <==
\begin{table}[!t]  
    \vspace{2.2mm}
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
        Latencies of different networking primitives (in $\mu$s) 
        on various NICs using an 8B payload. 
        For \emph{RDMA} and \emph{SNIC-H}, the CLI communicates with the SRV using 
        ConnectX-6 and Bluefield-2, respectively. 
        \emph{SNIC-S} means CLI  communicates with the on-board SoC of the SmartNIC. 
        }}}        
        \label{tab:lat-data}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
        \small{            
          \resizebox{.40\textwidth}{!}{%
          \begin{tabular}{lccc}
            \toprule
              & READ & WRITE & SEND+RECV \\ \hline
     RDMA     & 1.89          & 1.03                 & 2.10         \\
     SNIC-H   & \red{2.30}    & \red{1.29}           & \red{2.64}         \\
     SNIC-S   & 1.99          & \red{1.35}           & \red{3.38}         \\
     \bottomrule
     \end{tabular}           
        }
        } % end small
\end{table}   

==> linefs.tex <==
\section{Improved {\snic}-based Filesystem}
\label{sec:linefs}

\subsection{Overview of {\linefs}}
\label{sec:linefs-overview}

\begin{figure}[!t]
\begin{minipage}{1\linewidth}
\vspace{-2mm}
\hspace{-8mm}
%\centering    
\includegraphics[scale=0.9]{figs2/linefs.pdf}  
\end{minipage} \\[5pt]
\begin{minipage}{1\linewidth}
\caption{\small{%
Overview of the file write paths of {\linefs}. 
$rate$ is defined as \texttt{compressed size} / \texttt{uncompressed size}. 
We omit the payloads for control path RDMA messages as they are trivial. 
}}
\label{fig:linefs}
\end{minipage} \\[-10pt]
\end{figure}

{\linefs}~\cite{linefs} is the state-of-the-art distributed file system using non-volatile memory (NVM) and {\snic}.
It aims to offload file replication to {\snic} to reduce host CPU usage,
which suits off-path {\snic} well thanks for its support for general-purpose computation offloading. 
The files are stored in NVM, 
which are also replicated using chain-replication~\cite{DBLP:conf/osdi/RenesseS04}. 

{\linefs} chooses a path that \emph{completely offloads the file replication task to the {\snic}} (\ding{194} + \ding{192}). 
{\fig{fig:linefs}} gives a simplified overview of writing $d$ bytes to a file with {\linefs}. 
First, the host issues an RPC to notify NIC SoC of the file replication. 
The SoC uses READ to transfer the data in large chunks to its local memory (\red{\ding{182}}), 
compress it, and then issue another RPC to the backup node's SoC to ask for replication. 
After receiving the request, the replica SoC initiates one READ to read the  
compressed data (\red{\ding{183}}), 
decompresses the received data,
and finally, WRITEs the decompressed data to the host memory to finish the replication (\red{\ding{184}}). 
Note that the compression is optional. 

This path has non-trivial SoC-host communication latency. 
LineFS applies pipeline parallelism to hide the it, 
but pipelining cannot mitigate the overuse of PCIe bandwidth of such path (see \textsection{\ref{sec:dataflow-3}}).
Therefore, {\linefs} fails to utilize the network bandwidth of {\snic},
which we describe in details in the next section. 

\subsection{Improve the design and implementation of {\linefs}}
\label{sec:linefs-opt}

\begin{figure}[!t]
  \hspace{-3mm}
  \centering 
  \includegraphics[scale=1.17]{data/study/linefs-analysis.pdf}  \\[-3pt]
      \begin{minipage}{1\linewidth}
        \caption{\small{%
        A theoretical analysis of the file replication bandwidth. 
        }}
      \label{fig:linefs-analysis}
      \end{minipage} \\[-15pt]
  \end{figure} 

\begin{figure*}[!t]
\hspace{-2mm}
\centering 
\includegraphics[scale=1.2]{data/study/linefs.pdf}  \\[-5pt]
\begin{minipage}{1\textwidth}
\caption{\small{%
The host CPU usage breakdown of {\linefs} (a). 
Write throughput scalability when replicas are idle (b) and busy (c).
\TODO{The data here is just a placeholder. }          
}}
\label{fig:linefs-data}
\end{minipage} \\[-15pt]
\end{figure*} 

\stitle{Offloading-only design is inefficient. }
As we have discussed in \textsection{\ref{sec:dataflow-3}}, 
transferring bulk data between from host to SoC is a killer for PCIe bandwidth. 
It may even become the performance bottleneck if the transferred data is sent out through SoC later. 

Denote the primary's PCIe limit (uni) as $P$ and the compression ratio as $rate$. 
The maximum file transfer bandwidth of {\linefs} ($d$) is smaller than
$\frac{P}{1 + rate}$, 
because each data packet must pass the \emph{PCIe1 out link} twice. 
As shown in {\fig{fig:linefs}}, 
one is from SoC to RNIC (\red{\ding{182}}, $d$ bytes) and another from SoC to the remote (\red{\ding{183}}, $d \times rate$ bytes). 
Take the hardware parameters of our testbed ($P=256\,Gbps$). 
If the compression is disabled ($rate = 1$), 
the theoretical limit of {\linefs}'s offloading-only design is 128\,Gbps, 
roughly half of the network and NVM write bandwidth (200\,Gbps)\footnote{\footnotesize{
  Each Intel Optane 2 NVM module supports 25.2\,Gbps write bandwidth, 
  currently a server supports at most 8 modules per-socket (201\,Gbps)~\cite{optane}.
}}. 
To avoid under-utilize the network,
the compression rate must be lower than 28\%, as shown in {\fig{fig:linefs-analysis}},
which we believe is not always possible considering a general-purpose distributed filesystem. 
Note that this is not an issue in it in {\linefs} original evaluations, 
\ie{they only evaluate under 25\,Gbps}. 
But we show is problematic under faster networks.

The host can directly write to the replica without offloading to better utilize the PCIe bandwidth, as shown in {\fig{fig:linefs}}.
A concern about this approach is the extra CPU resources used by the host. 
In fact, if compression is disabled, the host CPU usage is nearly the same as an offloading approach
because {\linefs} also applies various optimizations to save host CPU usage (see {\fig{fig:linefs-data}}). 
In other words, a non-offloading design can reach the network bandwidth (200\,Gbps) for most compression rates 
\emph{without incurring extra CPU costs compared to an offloading design}. 

\paragraph{Improved design: a hybrid offloading scheme. }
\TODO{change to choose the best path}
A non-offloading design is not optimal either: 
it can only achieve 200\,Gbps without incurring extra CPU to compress the file, 
which is lower than an offloading design if the compression ratio is smaller (see {\fig{fig:linefs-analysis}}). 
To achieve the best of both worlds, 
we selectively offload a portion of the file replication to the SoC, with data compressed. 
Other parts are replicated by the host without compression to save CPU usage. 

\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{0pt}
\setlength\parskip{.3\baselineskip}

The challenge of a hybrid approach is how to choose the portion to offload. 
If offloading too much data on the SoC, the PCIe bandwidth is wasted. 
If offloading too less, we fail to utilize the compression for reduce network transfer. 
Fortunately, we can deduce the amount of offloading required using a simple model.  
Let $H$ be the host's part for replication and $S$ be the part offloaded to the {\snic}. We want to maximize $H+S$. 
The restrictions of choosing $H$ and $S$ are: 
\begin{equation}
H + S + S \times ratio \leq P 
\label{eq:1}
\end{equation}
\vspace{-5pt}
\begin{equation}
H + S \times ratio \leq N
\label{eq:2}
\end{equation}
\noindent (\ref{eq:1}) comes from the limit of PCIe1:
host send $H$ bytes to NIC via PCIe1, 
while SoC requires two passes, one to READ $S$ bytes from host,
and one to transfer $S \times ratio$ bytes to the NIC. 
 (\ref{eq:2}) comes from the fact that the aggregated bytes sent by the host and SoC 
should be smaller than the network bandwidth. 

To maximize replication bandwidth, 
we need to fully utilize the network, 
i.e., 
$H + S \times ratio = N$. 
Hence, we have: 
\begin{equation}
S \leq P - N
\end{equation}

\noindent
This formula not surprisingly matches our takeaway summarized in \textsection{\ref{sec:dataflow-together}}. 
Empirically, we found $S = P - N$ (56\,Gbps) is a good fit for $S$,
i.e., we only offload to SoC with \ding{194} if PCIe has bandwidth left. 
As shown in {\fig{fig:linefs-analysis}}, a hybrid design with such a choice 
can always beat the offloading only and non-offloading design for all the data compression ratio in theory. 

\subsection{Evaluation results}  
\label{sec:eval-linefs}

\stitle{Evaluation setup. }
We implement our hybrid approach upon LineFS's open-sourced codebase. 
The system configurations are tuned for the best throughput according to the author suggestions: 
\TODO{xx}

Since we don't have NVM, we emulate it with DRAM:
the current NVM's write bandwidth is larger than the network, 
so with properly configurations and optimizations, 
RNIC/SNIC can READ/WRITE NVM like ordinary DRAM~\cite{DBLP:conf/usenix/WeiX00Z21, DBLP:conf/cloud/KaliaAK20}. 

\stitle{Results. }
\TODO{xx}



==> overview-tab.tex <==
\begin{table*}[!ht]  
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
          A summary of whether {\snic} offload can accelerate different phases of RDMA-enabled distributed transactions.           
          \textbf{INW} (In-network wait) and \textbf{INI} (In-network install)
          are two techniques for offloading. \XD{RDMA-opt is not precise here.} 
        }}}
        \label{tab:overview}
        \end{minipage} %\\[2pt]  
        \ra{1.4}
%        \small{            
          \resizebox{1.\textwidth}{!}{%
\begin{tabular}{l|cccccccc}
                  & \textbf{Time(R)} & \textbf{Execution} & \textbf{Lock} & \textbf{Time(W)} & \textbf{Validation} & \textbf{Logging} & \textbf{Commit} & \textbf{Truncate}  \\ \hline
  %\textbf{RDMA-opt} & -                & One-sided          & Two-sided     & -                & One-sided           & One-sided        & Two-sided       & Two-sided          \\
\textbf{\snic-insight}  & Compute  & Bandwidth           &  \xmark   & Compute         &    \xmark                & \xmark           & \xmark          & Compute \\ %\hline  
\textbf{\snic-opt}  & INW (\textsection{\ref{sec:inw}})  & INC (\textsection{\ref{sec:inc}})            &  \xmark   & INW (\textsection{\ref{sec:inw}})          &    \xmark                & \xmark           & \xmark          & INI (\textsection{\ref{sec:ini}}) \\ \hline
\end{tabular}       
        }
%        }
%\\[-15pt]
\end{table*}         


==> overview.tex <==
\section{Optimization Space and Challenges}
\label{sec:overview} 

\input{overview-tab.tex}

\subsection{Offloading opportunities and challenges}

{\snic} has the following two drawbacks that are challenging for offloading 
phases in RDMA-enabled transactions~\cite{}: 

\paragraph{1. Wimpy NIC cores. }
\TODO{Describe what wimpy core means. }
In the context of transactions, \TODO{xx}.

\paragraph{2. Huge PCIe latency. }
\TODO{xx}

\input{snic-perf.tex}


\subsection{Existing SNIC-enabled solutions are not sufficient}

Xenic~\cite{xenic} is the only SmartNIC-accelerated RDMA-enabled distributed transaction. 
However, Xenic is designed for \TODO{on-path NIC}. 
Most techniques are in-applicable to our off-path SmartNICs. 


==> pcie-packet-tab.tex <==
\begin{table}[!t]  
    \vspace{2.2mm}
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
        The number of packets required for transferring $D$ bytes through PCIe links on {\snic}.
        Our simplified model omits control path packets (e.g., packets to notify the two-sided message arrival). 
        }}}        
        \label{tab:pcie-packet-mumber}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
        \small{            
          \resizebox{.48\textwidth}{!}{%
\begin{tabular}{l|ccc}
               \toprule
               & \textbf{SNC->Host (\ding{192})} & \textbf{SNIC->SoC (\ding{193})} & \textbf{SoC->Host (\ding{194})} \\ \hline
\textbf{PCIe1} &    $\lceil D/P_{host}\rceil$    &  0                              &   $\lceil D/P_{host}\rceil + \lceil D/P_{soc}\rceil $   \\
\textbf{PCIe0} &    $\lceil D/P_{host}\rceil$    &  $\lceil D/P_{soc}\rceil$       &   $\lceil D/P_{host}\rceil$                             \\
               \bottomrule
\end{tabular}
          }
        } % end small    
\end{table}  
%\vspace{-5pt}

==> pcie-payload-tab.tex <==
\begin{table}[!t]  
    \vspace{2.2mm}
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
        Maximum transfer unit (MTU) of different hardware.
        }}}        
        \label{tab:pcie-payload}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
        \small{            
          \resizebox{.48\textwidth}{!}{%
\begin{tabular}{l|cc}
              \toprule 
                             & \textbf{To Host CPU ($P_{host}$)}  & \textbf{To SoC CPU ($P_{soc}$)} \\ \hline
\textbf{PCIe MTU supported}  & 512B               & 128B         \\
              \bottomrule
\end{tabular}   
          }
        } % end small    
\end{table}  
%\vspace{-5pt}

==> phases-tab.tex <==
\begin{table}[!t]  
    \vspace{2.2mm}
    \centering    
    \begin{minipage}{1\linewidth}
      \caption{{\small{
        A summary of which RDMA primitive each system uses to accelerate a distributed transaction's phases.          
        \{\}+\{\} means using \{\} for locking and \{\} for reading during the validation phase.
        \{\}/\{\} means a hybrid choice. 
%        {\one} and {\two} stands for one-sided and two-sided primitives. 
        }}}        
        \label{tab:bg-rdma-tx-phases}
        \end{minipage} %\\[2pt]  
        \ra{1.2}
%        \small{            
          \resizebox{.48\textwidth}{!}{%
          \begin{tabular}{lccccc}
            \toprule
            \multicolumn{1}{c}{} &                        E        & V              & L      & C    & T \\ \hline
            FaRM~\cite{farm-v1,farm-v2}                 & One      & Two + One      & One    & Two  & Two  \\
            DrTM+R~\cite{drtmr}                         & One      & One + One      & One    & One  & Two  \\
            FaSST~\cite{fasst}                          & Two      & Two + Two      & Two    & Two  & Two  \\
            DrTM+H~\cite{drtm-h}                        & One/Two  & One/Two + One  & One    & Two  & Two  \\ 
            \bottomrule
            \end{tabular} 
        }
\end{table}    

==> snic-perf.tex <==
\begin{table}[!htb]
  \centering
  \begin{minipage}{1\linewidth}
        \caption{{\small{
		RDMA vs. {\dpu} when accessing the host's DRAM via one-sided RDMA READ. 
	}}}
	\label{tab:dpu-perf}
	\end{minipage} %\\[2pt]

	\resizebox{.48\textwidth}{!}{%
	\ra{1.2}
    \begin{minipage}{.5\linewidth}
%      \centering
    \small{
	  \begin{tabular}{l|ll}
   \textbf{In-rack}	& \textbf{Host} & \textbf{\snic} \\ \hline
   \textbf{Host}      &      &     \\
   \textbf{\snic}     &      &     \\
   \hline
   \end{tabular}	
    }
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
      \small{
	  \begin{tabular}{l|ll}
   \textbf{Cross-rack}	& \textbf{Host} & \textbf{\snic} \\ \hline
   \textbf{Host}      &      &     \\
   \textbf{\snic}  &      &     \\
   \hline
   \end{tabular}	
      }
    \end{minipage} 
	}
\end{table}

